More PAC-Bayes bounds: From bounded losses, to losses with general tail behaviors, to anytime validity

In this paper, we present new high-probability PAC-Bayes bounds for different types of losses. Firstly, for losses with a bounded range, we recover a strengthened version of Catoni's bound that holds uniformly for all parameter values. This leads to new fast-rate and mixed-rate bounds that are interpretable and tighter than previous bounds in the literature. In particular, the fast-rate bound is equivalent to the Seeger--Langford bound. Secondly, for losses with more general tail behaviors, we introduce two new parameter-free bounds: a PAC-Bayes Chernoff analogue when the loss' cumulative generating function is bounded, and a bound when the loss' second moment is bounded. These two bounds are obtained using a new technique based on a discretization of the space of possible events for the ``in probability'' parameter optimization problem. This technique is both simpler and more general than previous approaches optimizing over a grid on the parameters' space. Finally, using a simple technique that is applicable to any existing bound, we extend all previous results to anytime-valid bounds.

==> macros.tex <==

\definecolor{orange}{rgb}{1,0.4,0.0}

\newcommand{\ag}[1]{\textcolor{blue}{{#1}}}
\newcommand{\brg}[1]{\textcolor{orange}{{#1}}}
\newcommand{\todo}[1]{\textcolor{orange}{[{#1}]}}

\DeclarePairedDelimiterXPP{\KL}[2]{D_\textnormal{KL}}{(}{)}{}{%
#1\:\delimsize\|\:#2%
}
\DeclarePairedDelimiterXPP{\RD}[2]{D_{$\alpha$}}{(}{)}{}{%
#1\:\delimsize\|\:#2%
}

\DeclarePairedDelimiterXPP\Prob[1]{\mathbb{P}}{\lbrace}{\rbrace}{}{
\newcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}


\DeclarePairedDelimiterXPP{\lnorm}[2]{}{\lVert}{\rVert}{_{#2}}{#1}

\newcommand{\TV}{\ensuremath{\textsc{\texttt{TV}}}}
\newcommand{\MERln}{\ensuremath{\textsc{MER}_l^n}}
\newcommand{\MBR}{\ensuremath{\textsc{MBR}_r^T}}
\newcommand{\gen}{\ensuremath{\textnormal{gen}}}
\newcommand{\Egen}{\ensuremath{\bar{\textnormal{gen}}}}

\newcommand{\bA}{\ensuremath{\mathbb{A}}}
\newcommand{\bB}{\ensuremath{\mathbb{B}}}
\newcommand{\bC}{\ensuremath{\mathbb{C}}}
\newcommand{\bD}{\ensuremath{\mathbb{D}}}
\newcommand{\bE}{\ensuremath{\mathbb{E}}}
\newcommand{\bF}{\ensuremath{\mathbb{F}}}
\newcommand{\bG}{\ensuremath{\mathbb{G}}}
\newcommand{\bH}{\ensuremath{\mathbb{H}}}
\newcommand{\bI}{\ensuremath{\mathds{1}}}
\newcommand{\bJ}{\ensuremath{\mathbb{J}}}
\newcommand{\bK}{\ensuremath{\mathbb{K}}}
\newcommand{\bL}{\ensuremath{\mathbb{L}}}
\newcommand{\bM}{\ensuremath{\mathbb{M}}}
\newcommand{\bN}{\ensuremath{\mathbb{N}}}
\newcommand{\bO}{\ensuremath{\mathbb{O}}}
\newcommand{\bP}{\ensuremath{\mathbb{P}}}
\newcommand{\bQ}{\ensuremath{\mathbb{Q}}}
\newcommand{\bR}{\ensuremath{\mathbb{R}}}
\newcommand{\bS}{\ensuremath{\mathbb{S}}}
\newcommand{\bT}{\ensuremath{\mathbb{T}}}
\newcommand{\bU}{\ensuremath{\mathbb{U}}}
\newcommand{\bV}{\ensuremath{\mathbb{V}}}
\newcommand{\bW}{\ensuremath{\mathbb{W}}}
\newcommand{\bX}{\ensuremath{\mathbb{X}}}
\newcommand{\bY}{\ensuremath{\mathbb{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbb{Z}}}

\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cB}{\ensuremath{\mathcal{B}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\cE}{\ensuremath{\mathcal{E}}}
\newcommand{\cF}{\ensuremath{\mathcal{F}}}
\newcommand{\cG}{\ensuremath{\mathcal{G}}}
\newcommand{\cH}{\ensuremath{\mathcal{H}}}
\newcommand{\cI}{\ensuremath{\mathcal{I}}}
\newcommand{\cJ}{\ensuremath{\mathcal{J}}}
\newcommand{\cK}{\ensuremath{\mathcal{K}}}
\newcommand{\cL}{\ensuremath{\mathcal{L}}}
\newcommand{\cM}{\ensuremath{\mathcal{M}}}
\newcommand{\cN}{\ensuremath{\mathcal{N}}}
\newcommand{\cO}{\ensuremath{\mathcal{O}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\cS}{\ensuremath{\mathcal{S}}}
\newcommand{\cT}{\ensuremath{\mathcal{T}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cV}{\ensuremath{\mathcal{V}}}
\newcommand{\cW}{\ensuremath{\mathcal{W}}}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cY}{\ensuremath{\mathcal{Y}}}
\newcommand{\cZ}{\ensuremath{\mathcal{Z}}}

\newcommand{\ccA}{\ensuremath{\mathscr{A}}}
\newcommand{\ccB}{\ensuremath{\mathscr{B}}}
\newcommand{\ccC}{\ensuremath{\mathscr{C}}}
\newcommand{\ccD}{\ensuremath{\mathscr{D}}}
\newcommand{\ccE}{\ensuremath{\mathscr{E}}}
\newcommand{\ccF}{\ensuremath{\mathscr{F}}}
\newcommand{\ccG}{\ensuremath{\mathscr{G}}}
\newcommand{\ccH}{\ensuremath{\mathscr{H}}}
\newcommand{\ccI}{\ensuremath{\mathscr{I}}}
\newcommand{\ccJ}{\ensuremath{\mathscr{J}}}
\newcommand{\ccK}{\ensuremath{\mathscr{K}}}
\newcommand{\ccL}{\ensuremath{\mathscr{L}}}
\newcommand{\ccM}{\ensuremath{\mathscr{M}}}
\newcommand{\ccN}{\ensuremath{\mathscr{N}}}
\newcommand{\ccO}{\ensuremath{\mathscr{O}}}
\newcommand{\ccP}{\ensuremath{\mathscr{P}}}
\newcommand{\ccQ}{\ensuremath{\mathscr{Q}}}
\newcommand{\ccR}{\ensuremath{\mathscr{R}}}
\newcommand{\ccS}{\ensuremath{\mathscr{S}}}
\newcommand{\ccT}{\ensuremath{\mathscr{T}}}
\newcommand{\ccU}{\ensuremath{\mathscr{U}}}
\newcommand{\ccV}{\ensuremath{\mathscr{V}}}
\newcommand{\ccW}{\ensuremath{\mathscr{W}}}
\newcommand{\ccX}{\ensuremath{\mathscr{X}}}
\newcommand{\ccY}{\ensuremath{\mathscr{Y}}}
\newcommand{\ccZ}{\ensuremath{\mathscr{Z}}}

\newcommand{\mi}{\textup{I}}
\newcommand{\ent}{\textup{H}}
\newcommand{\relent}{\textup{D}}
\newcommand{\relentber}{\textup{d}}
\newcommand{\tv}{\textup{TV}}


\newcommand{\poprisk}[1]{\ccR(#1)}
\newcommand{\emprisk}[2]{\widehat{\ccR}(#1,#2)}

\newcommand{\stack}[2]{\stackrel{\mathclap{(#1)}}{#2}}

\newcommand{\indep}{ {\perp\!\!\!\perp} }

\newcommand{\defined}{{\stackrel{\mathclap{\textnormal{\tiny{def}}}}{=}}}

\newtheoremstyle{mytheoremstyle} %
    {\topsep}                    %
    {\topsep}                    %
    {\itshape}                   %
    {}                           %
    {\bf}                        %
    {.}                          %
    {.5em}                       %
    {}  %

\newcommand\xqed[1]{%
  \leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
  \quad\hbox{#1}}
  
\newcommand\symbolremark{\xqed{$\triangle$}}
\newcommand\symboldefinition{\xqed{$\diamond$}}

\DeclareMathOperator*{\esssup}{ess\,sup}

\theoremstyle{mytheoremstyle}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{example}{Example}

